Scheduling and Power Control for V2V Broadcast Communications with Co-Channel and Adjacent Channel Interference

This paper investigates how to mitigate the impact of both co-channel interference and adjacent channel interference (ACI) on vehicle-to-vehicle (V2V) broadcast communication by scheduling and power control. The optimal joint scheduling and power control problem, with the objective to maximize the number of connected vehicles, is formulated as a mixed integer programming problem with a linear objective and a quadratic constraint. From the joint formulation, we derive (a) the optimal scheduling problem for fixed transmit powers as a Boolean linear programming problem and (b) the optimal power control problem for a fixed schedule as a mixed integer linear programming problem. Optimal schedules and power values can, for smaller-size instances of the problem, be computed by solving first (a) and then (b). To handle larger-size instances of the problem, we propose heuristic scheduling and power control algorithms with reduced computational complexity. Simulation results indicate that the heuristic scheduling algorithm yields significant performance improvements compared to the baseline block-interleaver scheduler and that performance is further improved by the heuristic power control algorithm. Moreover, the heuristic algorithms perform close to the optimal scheme for small instances of the problem.

==> Drawings/OBI_schedulingMatrix_Utilda.tex <==
%\documentclass[varwidth,tikz,border=5pt]{standalone}
%\usetikzlibrary{matrix}
%\begin{document}


\tikzset{
	table/.style={
		matrix of nodes,
		row sep=-\pgflinewidth,
		column sep=-\pgflinewidth,
		nodes={
			rectangle,
			draw=black,
			align=center,
			text width = 0.4cm,    %%% adjust this
			minimum height=0.3cm,
			anchor=south,
			%        text depth=0.5ex,
			%        text height=2ex,
		},
		nodes in empty cells,
		row 1 column 1/.style={
			nodes={fill=gray!30}
		},
		row 1 column 2/.style={
			nodes={fill=gray!30}
		},
		row 1 column 3/.style={
			nodes={fill=gray!30}
		},
		row 2 column 1/.style={
			nodes={fill=gray!30}
		},
		row 2 column 2/.style={
			nodes={fill=gray!30}
		},
		row 3 column 3/.style={
			nodes={fill=gray!30}
		},
		row 3 column 1/.style={
			nodes={fill=gray!30}
		},
		row 3 column 2/.style={
			nodes={fill=gray!30}
		}
	}
}
\begin{tikzpicture}

\matrix (mat) [table]
{
	$1$ & $2$ & $3$ \\
	$7$ & $8$ & $0$ \\
	$4$ & $5$ & $6$ \\
	%		
	%		
	%		SO  & $f(x,y,z)$, $g(a,b,c)$, & & & &  &\\
	%		& AS    & B
	%		& C         & D & & \\
	%		2       & F         & 3D & H & J&&  \\
	%		3       & A         & B & DS & D&& \\
	%		4       & F         & G & H & 4D &&\\
	%		5       & F         & G & H & I & PS& \\
	%		6       & F         & G & H & I & & 4D\\
};
%	\begin{scope}
%	\draw[latex-] ([xshift=5ex]first-2-3.west)--([xshift=-5ex]first-2-2.east);
%	\draw[-latex] ([xshift=-5ex]first-2-3.east) -- ++(4ex,0) |- ([xshift=-5ex]first-3-3.east) ;
%	\end{scope}
\def\a{1.1cm}
\def\b{0.6cm}
%\draw[ <->] (-\a,-\b) -- (-\a,\b);
%\node[rotate=90] (RB) at (-1.4cm, 0) {$\fa$};
\def\a{1.1cm}
\def\a{0.9cm}
\draw[->] (-1.1,0.8) -- (1,0.8);
\node (RB) at (0,1cm) {timeslots};

\end{tikzpicture}
%\end{document}

==> Drawings/naturalSchedulingMatrix_Utilda.tex <==
%\documentclass[varwidth,tikz,border=5pt]{standalone}
%\usetikzlibrary{matrix}
%\begin{document}


\tikzset{
	table/.style={
		matrix of nodes,
		row sep=-\pgflinewidth,
		column sep=-\pgflinewidth,
		nodes={
			rectangle,
			draw=black,
			align=center,
			text width = 0.4cm,    %%% adjust this
			minimum height=0.3cm,
			anchor=south,
			%        text depth=0.5ex,
			%        text height=2ex,
		},
		nodes in empty cells,
		row 1 column 1/.style={
			nodes={fill=gray!30}
		},
		row 1 column 2/.style={
			nodes={fill=gray!30}
		},
		row 1 column 3/.style={
			nodes={fill=gray!30}
		},
		row 2 column 1/.style={
			nodes={fill=gray!30}
		},
		row 2 column 2/.style={
			nodes={fill=gray!30}
		},
		row 2 column 3/.style={
			nodes={fill=gray!30}
		},
		row 3 column 1/.style={
			nodes={fill=gray!30}
		},
		row 3 column 2/.style={
			nodes={fill=gray!30}
		}
	}
}
\begin{tikzpicture}

\matrix (mat) [table]
{
	$1$ & $2$ & $3$ \\
	$4$ & $5$ & $6$ \\
	$7$ & $8$ & $0$ \\
	%		
	%		
	%		SO  & $f(x,y,z)$, $g(a,b,c)$, & & & &  &\\
	%		& AS    & B
	%		& C         & D & & \\
	%		2       & F         & 3D & H & J&&  \\
	%		3       & A         & B & DS & D&& \\
	%		4       & F         & G & H & 4D &&\\
	%		5       & F         & G & H & I & PS& \\
	%		6       & F         & G & H & I & & 4D\\
};
%	\begin{scope}
%	\draw[latex-] ([xshift=5ex]first-2-3.west)--([xshift=-5ex]first-2-2.east);
%	\draw[-latex] ([xshift=-5ex]first-2-3.east) -- ++(4ex,0) |- ([xshift=-5ex]first-3-3.east) ;
%	\end{scope}
\def\a{1.1cm}
\def\b{0.6cm}
%\draw[ <->] (-\a,-\b) -- (-\a,\b);
%\node[rotate=90] (RB) at (-1.4cm, 0) {$\fa$};
\def\a{1.1cm}
\def\a{0.9cm}
\draw[->] (-1.1,0.8) -- (1,0.8);
\node (RB) at (0,1cm) {timeslots};


\end{tikzpicture}
%\end{document}

==> mypreamble.tex <==
\usepackage{cite}
\usepackage[cmex10]{amsmath}
\usepackage{amssymb}
\usepackage{mathtools}
\usepackage{amsthm,thmtools}
\usepackage{url}
\usepackage[dvipsnames]{xcolor}
\usepackage{bm}
\usepackage{standalone}
\usepackage{enumitem}
\usepackage[yyyymmdd,hhmmss]{datetime}
%\usepackage{fontenc}[T1]
\input{patterntikz}   %% Anver: Commented here, and instead manually included it before including this file

\usepackage{silence}
\WarningFilter{glossaries}{}
\usepackage{glossaries}
%\input{acronymdefs}   %% Commented by Anver

% theorem definitions
\theoremstyle{remark}
\declaretheorem[name=Example,qed={\lower-0.3ex\hbox{$\triangle$}}]{example}

\declaretheoremstyle[
spaceabove=6pt, spacebelow=6pt,
headfont=\normalfont\bfseries,
notefont=\mdseries, notebraces={(}{)},
bodyfont=\normalfont,
postheadspace=1em,
numberwithin=section,
qed=$\blacktriangleleft$
]{lemmastyle}

\declaretheorem{lemma}
\declaretheorem{theorem}


\hyphenation{op-tical net-works semi-conduc-tor}

% Our own operators
\newcommand{\re}{\mathop{\mathrm{Re}}\nolimits}
\newcommand{\im}{\mathop{\mathrm{Im}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\E}{\mathop{\mathbb{E}}\nolimits}
\newcommand{\lr}[1]{\ensuremath{\left({#1}\right)}}%leftright paranthesis
\newcommand{\lrb}[1]{\left \lbrace {#1} \right \rbrace}
\newcommand{\set}[1]{\left \lbrace {#1} \right \rbrace}
\newcommand{\lrh}[1]{\left [ {#1} \right ]}
\newcommand{\der}[2]{\frac{d#2}{d#1}}
\newcommand{\qfunc}[1]{Q \left( #1 \right) }
\newcommand{\mymod}[2]{\text{mod}\left( #1,#2 \right)}
\newcommand{\rpm}{\sbox0{$1$}\sbox2{$\scriptstyle\pm$} \raise\dimexpr(\ht0-\ht2)/2\relax\box2 }


\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\eqnref}[1]{(\ref{#1})}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\todo}[1]{{\color{magenta}#1}}
\newcommand{\tblu}[1]{{\color{blue}#1}}
\newcommand{\tred}[1]{{\color{red}#1}}
\newcommand{\multiline}[1]{\begin{tabular}{@{}c@{}} #1 \end{tabular}} % @{} removes the spacing
\newcommand{\myalign}[1]{\begin{aligned} #1 \end{aligned}}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}  % package: mathtools
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor} % package: mathtools

\newcommand{\valf}{\bm{\alpha}}
\newcommand{\vpsi}{\bm{\psi}}
\newcommand{\vbet}{\bm{\beta}}

==> sec02b_problemFormulation.tex <==
\section{Joint Scheduling and Power Control} \label{sec:system_model}

\subsection{Constraints Formulations}
Let $H_{i,j}$ be the average channel power gain from VUE $i$ to VUE $j$. Hence, $H_{i,j}$ takes into account pathloss and large-scale fading between VUE $i$ and VUE $j$. 
%Our problem formulation assumes full-duplex communication. However, one can use the same problem formulation for half-duplex communication too, by simply setting higher values for self interference channel, i.e., $H_{i,i} = 1$.

Let $\mathbf{X} \in \{0,1\}^{N \times F \times T }$ be the scheduling matrix defined as follows,
\begin{equation}
X_{i,f,t} \triangleq \left\{ \begin{array}{rll}
1, & \parbox{5cm}{\raggedright if VUE $i$ is scheduled in RB $(f,t)$ } \\
0, & \parbox{5cm}{\raggedright otherwise} \\
\end{array} \right. 
\end{equation}
\reviewerA{ Since $\mathcal{T}_j$ is the set of intended transmitters for VUE $j$, we ensure that all the VUEs in $\mathcal{T}_j$ are scheduled in non-overlapping RBs, using the following constraint upon $\Xb$,
%\begin{align}
%\sum_{i = 1}^{N} X_{i,f,t} &\leq 1  &\forall f,\, t  \label{constraintnVUEsInAnRB}
%\end{align}
\begin{equation}
	\sum_{i \in \mathcal{T}_j} X_{i,f,t} \leq 1 + N(1-Y_{j,f,t}) \quad \forall j,\, f,\, t  \label{constraintnVUEsInAnRB}
\end{equation}
 where the Boolean variable $Y_{j,f,t}$ indicate if VUE $j$ is able to successfully receive the packet in RB $(f,t)$ or not. We will discuss more upon $Y_{j,f,t}$ in \eqref{Ydefinition}. However, note that the above constraint is redundant when $Y_{j,f,t}=0$, since we want to enforce this condition only for successfully receiving VUEs in the corresponding RBs.
}

Similarly, to ensure our assumption \ref{assumption7}), i.e., a VUE is scheduled to at most one RB in a timeslot, 
%\begin{align}
%\sum_{f = 1}^{F} X_{i,f,t} &\leq 1  &\forall i,\, t   \label{constraintnRBsForAVUE}
%\end{align}
\begin{align}
	\sum_{f = 1}^{F} X_{i,f,t} \leq 1  \quad \forall i,\, t   \label{constraintnRBsForAVUE}
\end{align}


%A standard way of formulating the scheduling problem to maximize the number of successful links would result in a complicated problem formulation as shown in Appendix \ref{Appendix:powerControlFormulation}. 

Formulating the joint scheduling and power control problem to maximize the number of successful links in terms of the received SINR for VUE $j$ on RB $(f, t)$ will allow us to state the problem as an MIQCP problem. This is done with the support of our assumption \ref{assumption6}) and \ref{assumption7}) (i.e., constraints (\ref{constraintnVUEsInAnRB}) and (\ref{constraintnRBsForAVUE})). In contrast, as shown in Appendix \ref{Appendix:powerControlFormulation}, a formulation using the SINR for specific transmitter-receiver pairs results in a problem that is harder to solve. 


Let us define $\mathbf{\Gamma} \in \{0,1\}^{N \times F \times T}$ with $\Gamma_{j,f,t}$ as the received SINR of VUE $j$ in RB $(f,t)$. Note that the total signal power $S_{j,f,t}$ and interference power $I_{j,f,t}$ received by VUE $j$ in RB $(f,t)$ can be computed as follows,

\reviewerA{
\begin{align}
  S_{j,f,t}   &   =\sum_{i \in \mathcal{T}_j}   X_{i,f,t} P_{i,t} H_{i,j}  \label{definitionS}~,   \\
I_{j,f,t} &= \sum_{k \in \Ns \setminus \mathcal{T}_j}  X_{k,f,t}  P_{k,t} H_{k,j}  \nonumber \\
    &\hspace*{0.5cm} +   \overset{F}{\underset{\substack{f' = 1 \\ f' \neq f}}{\sum}}  \sum_{k \in 1}^{N}  \acirf X_{k,f',t}  P_{k,t} H_{k,j} ~,  \label{definitionI}   
\end{align}
Note that, the first term in \eqref{definitionI} is CCI from non-neighbouring VUEs, and the second term is ACI from all transmitting VUEs.}
The matrix $\mathbf{P} \in \mathbb{R}^{N \times T }$ with $P_{i,t}$ being the transmit power of VUE $i$, if scheduled in timeslot $t$. The value of $P_{i,t}$ is constrained by maximum transmit power $\Pmax$, i.e.,
\begin{equation}
0 \leq P_{i,t} \leq  \Pmax \qquad \forall\,i,t  \label{constrPower}
\end{equation}


Following (\ref{definitionS})  and (\ref{definitionI}), we can compute $\Gamma_{j,f,t}$ as follows,
\begin{equation}
\hspace{-2em}\Gamma_{j,f,t} = \frac{ S_{j,f,t}} {\sigma^2 +   I_{j,f,t} },
\end{equation}
where $\sigma^2$ is the noise variance. 

For successful links, $\Gamma_{j,f,t} \geq \gammaT$, i.e., 
\reviewerA{ 
\begin{align}
&& \frac{ S_{j,f,t}} {\sigma^2 +   I_{j,f,t} } &\geq \gammaT   \\
&\Leftrightarrow& \frac{ S_{j,f,t}} {\sigma^2 +   I_{j,f,t} + S_{j,f,t}} &\geq \frac{\gammaT}{1+\gammaT}   \\
&\Leftrightarrow& S_{j,f,t} - \gammaTbar (I_{j,f,t} + S_{j,f,t})  &\ge \gammaTbar \sigma^2.   \label{constraintSingleLink1}
\end{align}
where $\gammaTbar = \frac{\gammaT}{1+\gammaT}$, and $(I_{j,f,t} + S_{j,f,t})$ is the total received power.}  However, it might not be possible to fulfill this condition for all receivers $j$ in all RBs $(f, t)$. To select which combinations of $j$, $f$, and $t$ to enforce this condition, we use matrix $\mathbf{Y}\in\{0,1\}^{N\times F\times T}$, where
\begin{equation}
\label{Ydefinition}
Y_{j,f,t} \triangleq
\begin{cases}
1, & \text{if \eqref{constraintSingleLink1} is enforced}\\
0, & \text{otherwise}
\end{cases}
\end{equation}

We can combine~\eqref{constraintSingleLink1} and~\eqref{Ydefinition} into a single constraint as
\begin{equation}
\label{constraintMatrix2}
S_{j,f,t} - \gammaTbar (I_{j,f,t} + S_{j,f,t})  \ge \gammaTbar
\sigma^2 - \eta(1-Y_{j,f,t})\qquad\forall j, f, t    
\end{equation}
where $\eta$ is a sufficiently large number to make~\eqref{constraintMatrix2} hold whenever $Y_{j,f,t}=0$, regardless of the schedule and power allocation. It is not hard to show that $\eta = \gammaTbar(NP^{\mathrm{max}}+\sigma^2)$ is sufficient. 


%Since our goal is to make $\Gamma_{j,f,t} \geq \gammaT$ for all links, we get the following constraint,
%
%\begin{equation}
% S_{j,f,t}   -    \gammaT  I_{j,f,t}  \geq \gammaT \sigma^2  \quad\quad  \forall\, j,f,t  \label{constraintSingleLink1}
%\end{equation}
%%\flushleft where $\Pb$ is a diagonal matrix with $P_{i,t}$ as the \ith diagonal element.
%
%However, it may not be possible to satisfy the above constraint for all the receivers $j$ in all RBs $(f,t)$. Therefore, let us represent the set of receivers and RBs $(j,f,t)$ for which the above constraint is fulfilled by using a matrix $\mathbf{Y} \in \{0,1\}^{N \times F \times T}$. In other words, $Y_{j,f,t}$ indicates if the packet received by VUE $j$ in RB $(f,t)$ is successful or not as follows,
%
%%However, it may not be possible to make all links SINR to equal or greater than $\gammaT$, therefore, we try to maximize the total number of links achieving the SINR target $\gammaT$ by introducing a new matrix $\mathbf{Y} \in \{0,1\}^{N \times F \times T}$. The matrix $\mathbf{Y}$ indicates if a link is successful or not in RB $(f,t)$ as follows,
%\begin{equation}
%Y_{j,f,t} \triangleq \left\{ \begin{array}{rll}
%1, & \parbox[t]{5cm}{When (\ref{constraintSingleLink1}) is satisfied} \\ %% TODO
%0, & \mbox{otherwise} \\
%\end{array} \right. 
%\end{equation}
%
%We can nullify the constraint in (\ref{constraintSingleLink1}) by subtracting a sufficiently large number $\eta = \gammaT(N\Pmax+\sigma^2) $ from the right hand side of (\ref{constraintSingleLink1}), whenever $Y_{j,f,t}=0$. That is, the constraint (\ref{constraintSingleLink1}) becomes,
%
%\begin{align}
%S_{j,f,t}   -    \gammaT  I_{j,f,t}  \geq \gammaT \sigma^2 - \eta(1-Y_{j,f,t}) \quad  \forall\, j,f,t  \label{constraintMatrix2}
%\end{align}


\vspace{1\baselineskip}
\subsection{Problem Formulation}
%%%%%%%%%%%%%%%%%%% Erik's addition
We define a link as a transmitter-receiver pair $(i,j)$, and we say that the link $(i,j)$ is successful if at least one transmission from VUE~$i$ to VUE~$j$ is successful during the scheduling interval, i.e., that the SINR condition (\ref{constraintSingleLink1}) is satisfied for at least one RB $(f,t)$ where $f\in\{1, 2, \ldots, F\}$ and $t\in\{1, 2, \ldots, T\}$. We introduce the matrix $\mathbf{Z}\in\{0,1\}^{N\times N}$, where, for all $i, j$,
\begin{align}
Z_{i,j} &\triangleq \min\{1,   \sum_{t=1}^T\sum_{f=1}^F X_{i,f,t}Y_{j,f,t}\}  \label{ZijDefinition} \\
&=
\begin{cases}
1, & \text{link $(i,j)$ is successful}     \\
0, & \text{otherwise}
\end{cases}   
\end{align}
We note that the minimum in~\eqref{ZijDefinition} is required to not count successful links between VUE~$i$ and VUE~$j$ more than once.

The overall goal is to maximize the number of connected VUE pairs, i.e., to maximize the objective function
\begin{equation}
\label{jointProblemStatement}
J(\mathbf{X}, \mathbf{Y}, \mathbf{P})\triangleq \sum_{i=1}^N\sum_{\substack{j=1\\j\neq i}}^N Z_{i,j}
\end{equation}
subject to the constraints (\ref{constraintnVUEsInAnRB}), (\ref{constraintnRBsForAVUE}), (\ref{constrPower}), (\ref{constraintMatrix2}), and (\ref{ZijDefinition}). However, since $J$ is nonlinear in the binary matrices $\mathbf{X}$ and $\mathbf{Y}$, direct optimization of $J$ is cumbersome. We will therefore formulate an equivalent optimization problem which is simpler to solve. To this end, let us define two auxiliary matrices $\mathbf{V}\in\mathbb{R}^{N\times N\times F\times T}$ and $\mathbf{W}\in\mathbb{R}^{N\times N}$, where, for all $i, j$,
\begin{align}
\label{definitionV}
V_{i,j,f,t} &\in\{v\in\mathbb{R}: v \le X_{i,f,t}, v\le Y_{j,f,t}\},\\
W_{i,j} &\in\{w\in\mathbb{R}: w \le 1, w\le \sum_{t=1}^T\sum_{f=1}^F V_{i,j,f,t}\}.  \label{definitionW}
\end{align}
Now, for any fixed $\mathbf{X}$, $\mathbf{Y}$, it follows from~\eqref{definitionV} that 
\begin{equation}
V_{i,j,f,t}^\star = \max V_{i,j,f,t} = \min\{X_{i,f,t},Y_{j,f,t}\} = X_{i,f,t}Y_{j,f,t}.  \label{defVstar}
\end{equation}
The last equality in the above equation follows from the fact that both $X_{i,f,t}$ and $Y_{j,f,t}$ are boolean.  Moreover, it follows from~\eqref{definitionW} and~\eqref{ZijDefinition} that if $V_{i,j,f,t} = V_{i,j,f,t}^\star$, then
\begin{equation}
 \max W_{i,j} = \min\{1,\sum_{t=1}^T\sum_{f=1}^F V^{\star}_{i,j,f,t}\} = Z_{i,j}.  
\end{equation}

Hence, for any fixed $\mathbf{X}$, $\mathbf{Y}$, $\mathbf{P}$ we can compute $J(\mathbf{X}, \mathbf{Y}, \mathbf{P})$ as the optimal value of objective of 
\begin{maxi!}
	{\mathbf{V}, \mathbf{W}}{\sum_{i=1}^N \sum_{\substack{j=1\\ j\neq i}}^N W_{i,j}}
	{\label{eq:7}}{J(\mathbf{X}, \mathbf{Y}, \mathbf{P}) =}
	\addConstraint{\eqref{definitionV}, \eqref{definitionW}} \nonumber
\end{maxi!}

Putting everything together, we arrive at the optimization problem   
	\begin{subequations} \label{blp}
	\begin{align}
	&\ \max\limits_{\mathlarger{\mathbf{P},\Xb,\mathbf{Y},\mathbf{V},\mathbf{W}}}  \overset{N}{\underset{i=1}{\sum}}  \overset{N}{\underset{\substack{j=1, \\ j \neq i} } {\sum}}  W_{i,j}  \label{blp_obj} \\
	&\mbox{s.t. } \nonumber \\
	& \reviewerA{\underset{i \in \mathcal{T}_j}{\sum}}   X_{i,f,t} P_{i,t} H_{i,j}   - \reviewerA{\gammaTbar  \overset{F}{\underset{f' = 1}{\sum}}}  \overset{N}{\underset{k=1}{\sum}}  \acirf X_{k,f',t} P_{k,t} H_{k,j} \hspace*{1.5cm}    \nonumber \\
	&   \hspace*{0.2cm}\geq \gammaTbar \sigma^2 - \gammaTbar(N\Pmax+\sigma^2) (1-Y_{j,f,t}) \hspace*{0.3cm} \forall \, j,f,t    \label{blpConstr1} \\[5pt]    
	%%
	&W_{i,j}   \leq  \overset{T}{\underset{t=1}{\sum}} \overset{F}{\underset{f=1}{\sum}}    V_{i,j,f,t}  \hspace*{3.2cm}  \forall\, i,j   \\
	&W_{i,j} \leq 1 \hspace*{5cm}  \forall\, i,j  \\
	&V_{i,j,f,t} \leq X_{i,f,t}   \hspace*{4.1cm}   \forall\, i,j,f,t  \\
	&V_{i,j,f,t} \leq Y_{j,f,t}    \hspace*{4.2cm}  \forall\, i,j,f,t  \\
	%%			
	& \reviewerA{  \sum_{i \in \mathcal{T}_j} X_{i,f,t} \leq 1 + N(1-Y_{j,f,t})   \hspace*{1.6cm}   \forall\, j,\, f,\, t } \\
	&\sum_{f = 1}^{F} X_{i,f,t} \leq 1  \hspace*{4.3cm}   \forall\, i,\, t \\
	&\  0 \leq P_{i,t} \leq \Pmax   \hspace*{4cm}  \forall\, i,t  \\				
	&\mathbf{X},\mathbf{Y} \in \{0,1\}^{N \times F \times T }	\label{blp_booleanConstr}  \hspace*{2.8cm} 	 \\
	&\Pb\in\mathbb{R}^{N\times T} \\
	&\mathbf{V}\in\mathbb{R}^{N\times N\times F\times T} \\
	&\mathbf{W}\in\mathbb{R}^{N\times N}
	\end{align}
\end{subequations}

The above problem formulation allows for full-duplex
communication. Of course, if the self-channel power gain $H_{j,j}$ is
sufficiently large compared with the inter-VUE channel power gains $H_{i,j}$,
$i\neq j$, then (\ref{blp}) provides a half-duplex solution
for scheduling and power control, i.e., that a VUE cannot receive
packets at any RB $(f',t)$ while transmitting on RB $(f,t)$. However,
if the diagonal elements of $\mathbf{H}$ are very large compared to the
off-diagonal elements, this can cause numerical issues while
solving~(\ref{blp}). For this reason, when a half-duplex solution is implied
by $\mathbf{H}$ (or otherwise desired), it is better to explicitly enforce a
half-duplex solution by adding the constraint
\begin{equation}
Y_{j,f,t} \le 1 - X_{j, f', t}\qquad\forall j, f, f', t \tag{20n} \label{constrHalfDuplexCondition}
\end{equation}
and replacing $H_{i,j}$ with
$\tilde{H}_{i,j}$ in~(\ref{blpConstr1}), where
\begin{equation}
\tilde{H}_{i,j} = 
\begin{cases}
H_{i,j}, & i\neq j\\
0, & \text{otherwise}
\end{cases}
\end{equation}
Replacing $\mathbf{H}$ with $\tilde{\mathbf{H}}$ is done solely for
numerical reasons, since~(\ref{constrHalfDuplexCondition}) is sufficient to force the solution to
be half-duplex.   

We see that the problem~(\ref{blp}), in its full-duplex and half-duplex
formulation, has linear objective and constraints except the constraint (\ref{blpConstr1}), which is quadratic. We call such a problem a MIQCP problem.  Moreover, as shown in
Appendix~\ref{Appendix-nonConvexity}, the problem is nonconvex even after relaxing all the Boolean constraints, which will require a
sophisticated and complex solver \cite{Nesterov}. We will therefore not try to solve (\ref{blp})
directly, but will use it to find near-optimal schedules for fixed
transmit powers and near-optimal power allocation for fixed schedules
in Section IV-C and V-A, respectively.

\reviewerB{
As a side note, the problem formulation (\ref{blp}) can be translated into a problem to maximize the minimum number of successful links for a VUE, instead of total number of successful links. In this way, we are guaranteeing atleast $L^*$ successful links for any VUE. This is done by changing the objective function (\ref{blp_obj}) as follows,
\begin{equation}
L^* = \max\limits_{\mathlarger{\mathbf{P},\Xb,\mathbf{Y},\mathbf{V},\mathbf{W},L}}   L
\end{equation} 
and adding an extra constraint to (\ref{blp}) as follows,
\begin{equation}
\sum_{\substack{j=1 \\ j \neq i}}^{N}  Z_{i,j} \geq L  \qquad \forall\,i
\end{equation}
}

%The above problem formulation is for full-duplex communication. However, if the self-channel power gain $H_{i,i}$ is high enough, e.g., $H_{i,i}=1$, then (\ref{blp}) provides a half-duplex solution for scheduling and power control. However, setting high values for diagonal entries of channel matrix $\Hb$ makes the matrix ill-conditioned, thereby making (\ref{blp}) hard to solve. We can avoid this ill-conditioning by adding an extra constraint (\ref{constrHalfDuplex}) and by slightly modifying constraint (\ref{blpConstr1}) to (\ref{blpConstr1Modified}) as explained in Appendix \ref{Appendix-WellConditioning}. However, even after dropping the boolean requirements (\ref{blp_booleanConstr}), the above problem is nonconvex due to the nonconvex constraint (\ref{blpConstr1}) as proved in Appendix \ref{Appendix-nonConvexity}. Nonconvex MIQCP is harder to solve and requires more sophisticated global optimization techniques. We use the above problem formulation to find the near-optimal solution for scheduling and power control as explained in Sections \ref{subsec:NearOptimalScheduling} and \ref{subsec:nearOptimalPC}, respectively.






%%% Local Variables:
%%% mode: latex
%%% TeX-master: "Joint_Scheduling_and_PowerControl"
%%% End:

